Topic Sensitive Attention on Generic Corpora Corrects Sense Bias in Pretrained Embeddings

Given a small corpus $\mathcal D_T$ pertaining to a limited set of focused topics, our goal is to train embeddings that accurately capture the sense of words in the topic in spite of the limited size of $\mathcal D_T$. These embeddings may be used in various tasks involving $\mathcal D_T$. A popular strategy in limited data settings is to adapt pre-trained embeddings $\mathcal E$ trained on a large corpus. To correct for sense drift, fine-tuning, regularization, projection, and pivoting have been proposed recently. Among these, regularization informed by a word's corpus frequency performed well, but we improve upon it using a new regularizer based on the stability of its cooccurrence with other words. However, a thorough comparison across ten topics, spanning three tasks, with standardized settings of hyper-parameters, reveals that even the best embedding adaptation strategies provide small gains beyond well-tuned baselines, which many earlier comparisons ignored. In a bold departure from adapting pretrained embeddings, we propose using $\mathcal D_T$ to probe, attend to, and borrow fragments from any large, topic-rich source corpus (such as Wikipedia), which need not be the corpus used to pretrain embeddings. This step is made scalable and practical by suitable indexing. We reach the surprising conclusion that even limited corpus augmentation is more useful than adapting embeddings, which suggests that non-dominant sense information may be irrevocably obliterated from pretrained embeddings and cannot be salvaged by adaptation.

==> methods.tex <==
\section{Method}
The neighborhood (nearest words) for a word in the embedding space reflect the dominant sense of the word.
The crux of our method is based on the observation that we can analyze the neighborhood of a word in the source only embedding space and target only embedding space and detect if the dominant sense in source no longer aligns with the target. 
In the following section, we discuss in more detail the formulation we used to quantify this semantic drift.



\subsection{Sense Correction (Idea 1)}
\label{sec:wtd_avg}
We propose a simple trick to adapt the embeddings of the words that are observed to have drifted. 
For words that appear in both source and target, semantic drift score computed using expression~\ref{eqn:sem_drift} if greater than $\lambda$, a hyper-parameter, is considered to have changed in sense and is sense corrected. 
A word in the source corpus which is believed to have changed in sense is then replaced by a weighted average of the embeddings of closest neighbors for the word in target embedding space as shown in equation~\ref{eqn:correction}.
\begin{equation}
V^{new}(w) = V(w) + \Sigma_{n\in N_{target}(w)} V(n)*exp(-\gamma *R(n))
\label{eqn:correction}
\end{equation}
where $N_{target}(w)$ is used to denote the ordered list of neighbors for word \textit{w} in target, restricted to the top-k. 
R(n) denotes the rank of \textit{n} in this list.

Words that appear in only source but not in target are retained their vector representation from source as is\footnote{this slightly improved the performance}. 
Performance is observed to have degraded when including words that appear in target but not in source with their corresponding vector representation from vanilla adapted embedding, baseline (3) discussed in the baselines section.   

\subsection{Manipulating the co-occurrence matrix (Idea 2)}
\label{sec:idea_2}
A row in the co-occur matrix (pre-processing step of GloVe) captures co-occur frequency with other words in the vocabulary. 
We doctor the rows in a co-occur matrices to combine SRC and TGT whenever we are confident of a sense switch.
If we are confident of a sense switch, we distribute the total number of occurrences of the word (frequency in SRC + frequency in TGT) using the conditional distribution from the TGT.

Since the co-occurrence matrix is no longer symmetric and because we are only manipulating rows but not the columns of the source co-occurrence matrix, we consider only the focus vectors as the valid representation instead of any aggregation with the context vectors\footnote{We also tried and confirmed that context+focus vectors perform worse than using focus vectors alone}. 

\subsection{Regularization (Idea 3)}
Similar to the proposal in the \cite{Yang2017}, we can use the semantic drift scores as a regularization coefficient on the Skip-gram model.
We use the exact formulation proposed in the paper including the hyper-parameter search bounds with the only change that semantic drift score discussed in section~\ref{sec:sem_drift} is used instead of harmonic mean of normalized frequency of the word proposed in their paper. 

\subsection{Controlled source injection (Idea 4)}
When representations are learned over the combined source and target corpus, we risk getting target corpus dominated by the source corpus. 
For this reason, we carefully control the information from the source corpus. 
We define the frequency of a word in the mixed corpus as a weighted combination of frequency in source and the target while keeping the maximum frequency count from source capped at a small value (say 10) as shown below.

$$f_M(w) = \lambda*f_{src}(w) + f_{target}(w)$$

$f_{src}(w)$ and $f_{tgt}(w)$ are the source and target frequencies of the word \textit{w}.
A score is assigned to the words in the target vocabulary based on how much support the word has in the target corpus (frequency) and a measure of sense drift discussed in section~\ref{sec:sem_drift}.
We use the score so assigned to decide which of source or target context to use. 
The context for a given word \textit{w} in the mixed corpus is as shown below.

$$P_{M}(c|w) = (1-\alpha_s)*P_{src}(c|w) + \alpha_s*P_{tgt}(c|w)$$
$$\alpha_s = G(f_{tgt}(w), C_d[source\rightarrow target])$$

Finally, the loss on which the representations are learned is shown in expression \ref{exp:idea_4}.

\subsubsection{Technical Details}
For negative sampling, we tried sampling from the unigrams from SRC alone and from SRC and TGT when the sentence is drawn from source and target respectively. 
We found the best performance when negative sampling from unigram probability set to sum of frequencies in source and target, this gave a three point improvement over other variants. 

Also, we used the combined source and target frequency for words and this slightly improved the performance.

We tried different coarse schedules over the source and target and found training on all sentences from source followed by target and followed by source and so on to be best performing.

In the case of physics stack-exchange, F1 score improved by 2-3 points by not training representations of words in target but not in source and hence retaining their initial random vectors.  

Words with the target sense are trained only on target, as in the word is not considered a focus or a context word if the sentence is from source corpus. 
Words with source sense are trained on both source and target. 

Main steps:
\begin{enumerate}
\item Estimate mixed distribution vectors $P_M(c|w)$
\item Estimate joint co-occurrence $n_{cw}$ to minimize $P_{M}(w) KL(P_M(c|w); P_n(c|w)) + KL(P_{tgt}(w); P_n(w))$
\item Run skip-gram over joint co-occurrence.
\end{enumerate}

\subsection{Joint with document classification (Idea 5)}
If we learn embeddings for document classification using say an RNN, the target specific words are replaceable only with the target words which serves the purpose of retaining the correct sense for the words\footnote{I observed this empirically with a document classification model trained on Wikipedia and Physics stack exchange corpus, although the wiki text is 20 times bigger and dominates the target corpus, correct sense is reflected for the physics specific ambiguous words in their neighborhood and distances.}.
However, the embedding obtained by this model cannot be used for down-stream applications as is because they do not capture the semantics as accurately as a context predicting word representation.
Hence the proposal is to jointly train word vectors for document classification and context prediction.
Or perhaps we can just initialize embeddings from one task for the other and use the final embeddings. 

\cite{Joulin2016} uses a Continuous Bag of Words (CBoW) like model to predict the label of the document and have shown that this simple linear model can perform on par with other complex non-linear models. 
In \cite{ftclassify}, the focus word is replaced with the label to be predicted. 
We use a CBOW model to learn word representations and also to predict the label of the word. 
That is, for every context and focus word pair, we use the context to predict the focus word and also the origin of sentence -- source or target. 
Implementation wise, this only requires that we learn a vector corresponding to the source domain and to the target domain. 
Shown in the result tables are two variants of this method, when the vocabulary is learned from (1) both source and target corpus and (2) target corpus alone. 
Superior results are seen in the latter case.

The final objective is shown in expression~\ref{eq:joint}.
Other variants yet to be tried are shown in \ref{eq:var1}~\ref{eq:var2}~\ref{eq:var3}

\begin{equation}
\begin{split}
\mathcal{L} = \Sigma_{<w,c>\in SRC}[\sigma (v_w\cdot v_c) + \Sigma_{\tilde{w} \sim neg(V)} \sigma (-v_{\tilde{w}}\cdot v_c) \\
+ \lambda*(\sigma(v_{src}\cdot v_c) + \sigma(-v_{tgt}\cdot v_c))] \\
+ \Sigma_{<w,c>\in TGT}[\sigma (v_w\cdot v_c) + \Sigma_{\tilde{w}\sim neg(V)} \sigma (-v_{\tilde{w}}\cdot v_c) \\
+ \lambda*(\sigma(v_{tgt}\cdot v_c) 
+ \sigma(-v_{src}\cdot v_c))]\\
\end{split}
\label{eq:joint}
%\caption{Implemented and works}
\end{equation}

\begin{equation}
\begin{split}
\mathcal{L} = \Sigma_{<w,c>\in SRC}\alpha_s(w)[\sigma (v_w\cdot v_c) + \Sigma_{\tilde{w} \sim neg(V)} \sigma (-v_{\tilde{w}}\cdot v_c)] \\
+ \Sigma_{<w,c>\in TGT}[\sigma (v_w\cdot v_c) + \Sigma_{\tilde{w}\sim neg(V)} \sigma (-v_{\tilde{w}}\cdot v_c)]
\end{split}
\label{eq:var1}
\end{equation}

\begin{equation}
\begin{split}
\mathcal{L} = \Sigma_{<w,c>\in SRC}[\sigma (v_w\cdot v_c) + \Sigma_{\tilde{w} \sim neg(V)} \sigma (-v_{\tilde{w}}\cdot v_c) \\
+ \lambda*(\sigma(-v_{tgt}\cdot v_c))] \\
+ \Sigma_{<w,c>\in TGT}[\sigma (v_w\cdot v_c) + \Sigma_{\tilde{w}\sim neg(V)} \sigma (-v_{\tilde{w}}\cdot v_c) \\
+ \lambda*(\sigma(v_{tgt}\cdot v_c) )]\\
\end{split}
\label{eq:var2}
\end{equation}

\begin{equation}
\begin{split}
\mathcal{L} = \Sigma_{<w,c>\in SRC}\alpha_s(w)[\sigma (v_w\cdot v_c) + \Sigma_{\tilde{w} \sim neg(V)} \sigma (-v_{\tilde{w}}\cdot v_c) \\
%+ \sigma(v_{src}\cdot v_c) + 
+ \sigma(-v_{tgt}\cdot v_c)] \\
+ \Sigma_{<w,c>\in TGT}[\sigma (v_w\cdot v_c) + \Sigma_{\tilde{w}\sim neg(V)} \sigma (-v_{\tilde{w}}\cdot v_c) \\
+ \sigma(v_{tgt}\cdot v_c) 
%+ \sigma(-v_{src}\cdot v_c)]\\
\end{split}
\label{eq:var3}
\end{equation}

\textit{c} in expression~\ref{eq:cbow} refers to all the words in the context of the focus word: \textit{w} and $v_{(\cdot)}$ refers to the vector corresponding a word. 
$v_c$ is used to refer to the average of all the vectors in the context \textit{c}, that is $v_c=\frac{\Sigma_{c_w\in c}v_{c_w}}{\Sigma_{c_w\in c}1}$.
$v_{src}$ and $v_{tgt}$ correspond to the source and target vectors (weights) which are used for classification of a given context.
$neg(V)$ refers to unigram frequencies over the vocabulary: $V$ used for negative sampling. 

$\alpha_s(w)$ takes small values for words whose sense has drifted from source to target.

\subsection{Distant supervision (Idea 6)}

\subsection{Source selection (Idea 7)}
Train a snippet-level source Vs target classifier $P(T|w,c)$ on a sample of source and target snippets

For each source snippet $(w,c)$ assign a $p_{w,c} = P(T|w,c)$.

Learn embeddings with union of target and weighted source embeddings.  Weight of source snippet $(w,c)$ is $\lambda p_{w,c}$.  $\lambda$ is chosen to balance the relative contribution of source and target snippets.

We compare our approach with the following methods: 
(1) Embeddings calculated from the target corpus (TGT) 
(2) Embeddings calculated from the source corpus (SRC) 
(3) Vanilla adapted embeddings are estimated by initializing with SRC embeddings and re-training on target corpus (SRC INIT)
(4) Embeddings are trained on SRC + TGT corpus (SRC+TGT)
(5) Word vectors from SRC and TGT are concatenated over the words that appear in both source and target (concat)
(6) Skip-gram regularization method \cite{Yang2017}. 
(7) CBOW model regularized with drift score, similar to \cite{Yang2017}, shown in expression~\ref{eqn:drift_score} (CREG). 
(8) Skip-gram model regularized with score, similar to \cite{Yang2017}, shown in expression~\ref{eqn:drift_score} (SREG). 
(9) The down-stream task is initialized with target trained word vectors and are allowed to be trained, i.e. tweaked on the task (TT).

Idea 8 is context similarity with target trained vectors and threshold to select a context is mean + standard deviation from context similarity measures for each word in the target corpus.
Idea 9 is weighting of source contexts with $tanh(\lambda*CosSim(context))$.

% \begin{center}
% \begin{table}[h]
% \begin{tabular}{|l|rrr|}
% \hline
%  & F1 & Recall & Precision\\
% \hline
% % TGT & 0.765 & 0.687 & 0.865 \\
% SRC & 67.1 & 59.2 & 77.6 \\
% CONCAT & 64.0 & 53.9 & 81.7\\
% SRC+TGT & 71.2 & 61.1 & 85.9\\
% \cite{Yang2017} (sgram) & 65.3 & 59.8 & 72.0\\
% \cite{Yang2017} (cbow) & 72.6 & 68.1 & 77.9\\
% TGT & 70.4 & 61.4 & 82.7 \\
% Idea 1 & 73.5 & 68.9 & 78.7 \\
% Idea 12 & 75.0 & 68.4 & 83.4 \\
% % CONCAT & 0.722 & 0.632 & 0.862 \\
% % SRC+TGT & 0.746 & 0.689 & 0.815 \\
% % SRC INIT (CBOW) & 0.750 & 0.681 & 0.835 \\
% % SRC INIT (SGRAM) & 0.642 & 0.529 & 0.880 \\
% % CREG & 0.753 & 0.689 & 0.834 \\
% % SREG & 0.699 & 0.614 & 0.839 \\
% % TT & 0.767 & 0.712 & 0.833 \\
% % \cite{Yang2017} & 0.666 & 0.605 & 0.767\\
% % \textbf{Idea 6} & 0.777 & 0.711 & 0.857\\
% % \textbf{Idea 6 (asymmetric)} & 0.783 & 0.704 & 0.884\\
% % Idea 7 & 0.784 & 0.716 & 0.870 \\
% % Idea 8 & 0.780 & 0.714 & 0.863 \\
% % Idea 9 & 0.777 & 0.702 & 0.874 \\
% % Idea 10 & 0.770 & 0.704 & 0.852 \\
% % Idea 11 & 0.787 & 0.733 & 0.850 \\

% \hline
% \end{tabular}
% \label{tab:results_gaming}
% \caption{De-duplication results on Gaming Stack-exchange}
% \end{table}
% \end{center}

% \begin{center}
% \begin{table}[h]
% \begin{tabular}{|l|rrr|}
% \hline
%  & F1 & Recall & Precision\\
% \hline
% % TGT & 0.848 & 0.811 & 0.888\\
% % CONCAT & 0.774 & 0.701 & 0.868\\
% % SRC+TGT & 0.780 & 0.690 & 0.900\\
% % SRC INIT (CBOW) & 0.830 & 0.806 & 0.857 \\
% % SRC INIT (SGRAM) & 0.784 & 0.691 & 0.909 \\
% % CREG & 0.830 & 0.79 & 0.879 \\
% % SREG & 0.783 & 0.706 & 0.896 \\
% % \cite{Yang2017} & 0.796 & 0.719 & 0.897 \\
% % Idea 6 & 0.847 & 0.81 & 0.890 \\
% % Idea 6 (asymmetric) & 0.848 & 0.825 & 0.873 \\
% % Idea 7 & 0.852 & 0.807 & 0.904 \\
% % Idea 8 & 0.832 & 0.774 & 0.903 \\
% % Idea 9 & 0.851 & 0.812 & 0.893 \\
% % Idea 10 & 0.839 & 0.787 & 0.899 \\
% % Idea 11 & 0.839 & 0.790 & 0.898 \\
% SRC & 72.3 & 61.1 & 89.3\\
% SRC+TGT & & & \\
% CONCAT & & & \\
% TGT & 82.5 & 77.6 & 88.1 \\
% \cite{Yang2017} (cbow) & 83.8 & 80.5 & 87.4\\
% \cite{Yang2017}(sgram) & & & \\
% Idea 1 & 81.7 & 79.2 & 84.9 \\
% Idea 12 & 83.8 & 80.8 & 86.9 \\
% \hline
% \end{tabular}
% \label{tab:results_android}
% \caption{De-duplication results on Android Stack-exchange}
% \end{table}
% \end{center}

% \begin{center}
% \begin{table}[h]
% \begin{tabular}{|l|rrr|}
% \hline
%  & F1 & Recall & Precision\\
% \hline
% %TGT & 0.693 & 0.612 & 0.805 \\
% SRC & 46.6 & 34.1 & 74.9 \\
% SRC+TGT & & & \\
% CONCAT & & & \\
% TGT & 67.7 & 58.7 & 79.9 \\
% \cite{Yang2017}(cbow) & & & \\
% \cite{Yang2017}(sgram) & & & \\
% Idea 12 & 66.5 & 57.1 & 79.6 \\
% % CONCAT & 0.601 & 0.501 & 0.752 \\
% % SRC+TGT & 0.602 & 0.505 & 0.777 \\
% % SRC INIT (CBOW) & 0.698 & 0.645 & 0.767 \\
% % SRC INIT (SGRAM) & 0.665 & 0.643 & 0.707 \\
% % CREG & 0.700 & 0.629 & 0.791 \\
% % SREG & 0.631 & 0.622 & 0.689 \\
% % \cite{Yang2017} & 0.650 & 0.621 & 0.713 \\
% % Idea 6 & 0.692 & 0.607 & 0.805 \\
% % Idea 6 (asymmetric) & 0.689 & 0.595 & 0.817 \\
% % Idea 7 & 0.698 & 0.613 & 0.817 \\
% % Idea 8 & 0.693 & 0.595 & 0.829 \\
% % Idea 9 & 0.682 & 0.584 & 0.821 \\
% % Idea 10 & 0.697 & 0.615 & 0.806 \\
% % Idea 11 & 0.697 & 0.600 & 0.831 \\

% \hline
% \end{tabular}
% \label{tab:results_unix}
% \caption{De-duplication results on Unix Stack-exchange}
% \end{table}
% \end{center}






